TAPA: A Scalable Task-Parallel Dataflow Programming Framework for Modern FPGAs with Co-Optimization of HLS and Physical Design

In this paper, we propose TAPA, an end-to-end framework that compiles a C++ task-parallel dataflow program into a high-frequency FPGA accelerator. Compared to existing solutions, TAPA has two major advantages. First, TAPA provides a set of convenient APIs that allow users to easily express flexible and complex inter-task communication structures. Second, TAPA adopts a coarse-grained floorplanning step during HLS compilation for accurate pipelining of potential critical paths. In addition, TAPA implements several optimization techniques specifically tailored for modern HBM-based FPGAs. In our experiments with a total of 43 designs, we improve the average frequency from 147 MHz to 297 MHz (a 102% improvement) with no loss of throughput and a negligible change in resource utilization. Notably, in 16 experiments we make the originally unroutable designs achieve 274 MHz on average. The framework is available at https://github.com/UCLA-VAST/tapa and the core floorplan module is available at https://github.com/UCLA-VAST/AutoBridge.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart


PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)
SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx

samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	cd $(dir $@) && pdflatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex-dev $(notdir $<); done

samples/sample-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex-dev $(notdir $<)
	cd $(dir $@) && xelatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex-dev $(notdir $<); done

samples/sample-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all docclean
	zip -r $@ acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.*

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> backup/README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   \country is now obligatory for addresses.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> code/ring-hls.tex <==
\begin{tikzpicture}[font=\small,red,thick,overlay,remember picture]
  \node (a) at (pic cs:eot_top) {};
  \draw [decorate,decoration=brace] (a.north) -- (pic cs:eot_bottom)
    node [align=left,midway,right,xshift=1ex] {
      Auxiliary \texttt{struct} for termination control;\\
      \texttt{eot} stands for ``end of transaction''.
    };

  \node (a) at (pic cs:buf_top) {};
  \draw [decorate,decoration=brace] (a.north) -- (pic cs:buf_bottom)
    node [align=left,midway,right,xshift=1ex] {
      Manually maintained input\\
      buffers to implement non-\\
      destructive read (i.e., peek).
    };

  \node (a) at (pic cs:state_top) {};
  \draw [decorate,decoration=brace] (a.north) -- (pic cs:state_bottom)
    node [align=left,midway,right,xshift=1ex] {
      Manually\\update\\buffers.
    };
\end{tikzpicture}

\begin{listing}[!t]
  \begin{minted}[escapeinside=||,texcomments]{cpp}
    struct PktEoT { |\tikzmark{eot_top}\label{lln:eot_top}|
      Pkt pkt;
      bool eot;
    };              |\tikzmark{eot_bottom}\label{lln:eot_bottom}|
    void RingNode(stream<Pkt>& node_in,  stream<PktEoT>& pe_in,
                  stream<Pkt>& node_out, stream<Pkt>& pe_out) {
      Pkt node_pkt;                |\tikzmark{buf_top}\label{lln:peek_top}|
      bool node_pkt_valid = false;
      PktEoT pe_pkt;
      bool pe_pkt_valid = false;   |\tikzmark{buf_bottom}|
      while (!(|\colorpeek{pe\_pkt\_valid && pe\_pkt.eot}\label{lln:eot}|)) {
        if (!pe_pkt_valid)                            |\tikzmark{state_top}|
          pe_pkt_valid = pe_in.read_nb(pe_pkt);
        if (!node_pkt_valid)
          node_pkt_valid = node_in.read_nb(node_pkt); |\tikzmark{state_bottom}\label{lln:peek_bottom}|
        if (pe_pkt_valid) {
          node_out.write(|\colorread{pe\_pkt}|.pkt);
          |\colorread{pe\_pkt\_valid = false;}|
          if (node_pkt_valid && IsForThisNode(|\colorpeek{node\_pkt}|)) {
            pe_out.write(|\colorread{node\_pkt}|);
            |\colorread{node\_pkt\_valid = false;}|
          }
        } else if (node_pkt_valid) {
          Pkt pkt = |\colorread{node\_pkt}|;
          |\colorread{node\_pkt\_valid = false;}|
          (IsForThisNode(pkt) ? pe_out : node_out).write(pkt);
        }
      }  // Highlighted are \colorread{destructive read operations} and
    }    // \colorpeek{non-destructive read (peek) operations}.
  \end{minted}
  \caption{Ring network node written in Vivado HLS.}
  \label{lst:ring-hls-comm}
\end{listing}

\begin{listing}[!t]
  \begin{minted}[escapeinside=||]{cpp}
    void Kernel(...) {
      stream<Pkt, 2> node_0_1, node_1_2, ...
      stream<Pkt, 2> from_pe_0, to_pe_0, from_pe_1, to_pe_1, ...
      // Instantiates other channels...
    #pragma HLS dataflow
      RingNode(node_0_1, node_1_2, from_pe_1, to_pe_1);
      RingNode(node_1_2, node_2_3, from_pe_2, to_pe_2);
      // Instantiates other ring nodes and PEs...
    }
  \end{minted}
  \caption{Accelerator task instantiation in Vivado HLS.}
  \label{lst:ring-hls-inst}
\end{listing}


==> src/experiment.tex <==
\section{Experiments}
\label{sec:expriments}
% \begin{figure}[!h]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/flow.pdf}
%     \caption{Overall flow of AutoBridge.}
%     \label{fig:flow}
% \end{figure}

Based on the theoretical framework as introduced above, we implement an automated framework, AutoBridge, that works seamlessly with Vivado HLS and Xilinx Vitis / SDAccel tools to help programmers boost the frequency of their designs.

{Figure~\ref{fig:flow} presents the overview flow of AutoBridge.}
AutoBridge takes in the unmodified RTL outputs generated by Vivado HLS. Then it performs high-level floorplanning and introduces addition pipelining into the region-crossing signals as described in Section~\ref{sec:region assignment}. Next it re-balances the reconvergent paths to avoid the impacts on the design throughput, as presented in Section~\ref{sec:rebalance}. Lastly, AutoBridge generates the optimized RTL code and a constraint file specifying the floorplanning of the design to be used by Vivado. 
% In this section, we present our automated framework, AutoBridge, based on the previous theory. AutoBridge aims to 

At present, AutoBridge can automatically improve FIFO-based designs. As for shared-memory based designs, some steps still require manual help due to the difficulty of hacking HLS from the outside. We will leave the automation for these steps as the future work.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



\subsection{Implementation Details}
\label{sec:impl_details}
%\todo{I feel we need to have a background section about how Vivaod floorplanning works, and how AutoBrige is placed in the whole flow.}

Internally, AutoBridge analyzes various reports from HLS to extract the information about the design, such as the topology and the area of each module. To obtain how the module interacts with the external FIFO, AutoBridge analyzes the scheduling reports by HLS. %The scheduling report indicates which states belong to which pipelines, along with the operations in each state. Thus we can know which FIFOs are accessed in the same pipelined loop. 
For shared-memory-based designs, we analyze if the buffer accesses are inside the pipeline, thus determining whether we could add registers to them.

For FIFO-based designs, the only difference between our modified RTL and the original one is that some ordinary FIFOs will be replaced by our ``bridge'' units. The bridge directly adds registers to the FIFO ports, and makes use of the almost-full FIFO\footnote{Such FIFOs assert the \texttt{full} signal before the storage actually runs out.} to tolerate the additional latency, as shown in Figure~\ref{fig:relay_station}. Such simple modification to the RTL makes AutoBridge functionally robust.
The corresponding constraint file specifies a target region for each module. It also instructs the registers in our bridge units to spread with even distance. 
% So far our python-based tool can automatically handle the FIFO-based designs. {Jie: You have already mentioned it multiple places}

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/relay_station.pdf}
	\caption{Replace the ordinary FIFO by our ``bridge''}
    \label{fig:relay_station}
\end{figure}

Handling the shared-memory-based designs is more challenging than FIFO-based designs.
%easy in theory, but much harder in terms of engineering efforts. 
While we could directly add registers to the BRAM interface, we must adjust the internal logic of the design that relies on the fixed latency of the BRAM interface. Currently this task is performed manually. Specifically, we first insert an empty function in the source code, which will be compiled into a module that contains only one register by HLS. Then we relocate this register to the position where we want to add the latency. %Currently AutoBridge could only identify all the legal positions that we can add registers, but still relies on manual operations to add the register.

Additionally, AutoBridge exposes key parameters to users to customize according to their needs. For example, by default we allow up to 70\% of the resource of a region to be used to avoid local congestion. However, for very large designs, we can adjust the ratio accordingly. We are planning to automatically explore the best utilization ratio for each region, which remains as the future work. What's more, AutoBridge also allows users to annoate the location of specific modules according to their needs. 

Note that one crucial detail is that we must disable the hierarchy rebuild process during the synthesis step. This is because the hierarchy rebuilding process may blend signals across the module boundaries. As a result, if two interacting modules happen to be arranged far apart, while some of their internal signals are blended together, unexpected critical paths will show up in the generated design.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experiment Setup}

We evaluate our tool on two representative architectures: Alveo U250 FPGA and Alveo U280 HBM-based FPGA, as introduced in Section~\ref{sec:arch}. We select four large-scale real-world benchmarks, each with a different topology. The baseline is the original RTL generated by HLS, which is compared against our optimized RTL plus the floorplanning constraints. All experiments are performed using Vivado HLS 2019.2 and Xilinx Vitis 2019.2 with the highest level of optimization.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Stencil Computation (Line Topology)}

We use this benchmark to 1) motivate the idea of HLS-floorplanning co-design and 2) demonstrate the stability of the timing quality of designs optimized by AutoBridge. We use the SODA compiler~\cite{chi2018soda} to generate different accelerator designs.

\begin{itemize}
    \item The SODA compiler supports generating multiple kernels concatenated via FIFO interface. We adjust the size of our line-topology design by varying the number of kernels to observe how the frequency changes accordingly.
    
    \item The configuration details of SODA are as follow. We choose the Jacobi2D kernel, with tile size of 8000 and unroll factor of 64. For the HBM-based U280 FPGA, we choose the DRAM number of 4. The generated accelerator will read from 4 banks and write to 4 banks. For the U250 FPGA, we choose the DRAM number of 1. Figure~\ref{fig:soda_arch} shows the topology of the accelerator.
    
    \item The connections between the accelerator and the FPGA are as follow. On U280, we set all the inbound memory banks at the left side of the HBM IP, and outbound memory banks at the right side. On U250, we set the inbound DDR controller as the bottom one and the outbound DDR controller as the upper one.
    
    %\item AutoBridge automatically analyzes and optimizes this FIFO-based design witho.
\end{itemize}


 
\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/soda_arch.pdf}
	\caption{Topology of the SODA stencil computation accelerator.}
    \label{fig:soda_arch}
\end{figure}

Next, we demonstrate the advantages of floorplanning at the HLS stage. Figure~\ref{fig:soda_dcp} visualizes the implementation results of the accelerator with four concatenated kernels on U280. For this design, Vitis / Vivado failed routing even with the highest level of optimization.
\begin{itemize}
    \item We can observe that the architecture of the U280 FPGA is the same as depicted in Section~\ref{sec:arch}. All the HBM ports are at the bottom; the Vitis platform IP takes up the rightmost columns and there is a nontrivial gap in the middle. 
    \item Figure~\ref{fig:soda_dcp} reveals a sharp contrast between the designs with or without the AutoBridge floorplanning. In this figure, each color represents one Jacobi2D kernel. In the baseline design generated by Vivado, the 4 kernels are twisted together. Each kernel spans across the die boundary and the middle gap multiple times. In comparison, in the design optimized by AutoBridge as shown on the right, AutoBridge generates a clean cut among modules to ensure the local timing quality and adds additional pipelining on cross-region paths to ensure the global timing quality. 
    \item Note that the only differences between the original and the optimized designs are a few more registers on the FIFO ports and an efficient floorplan. 
\end{itemize}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/soda_dcp.png}
	\caption{Comparison of the default floorplan of the 4-kernel stencil accelerator on U280 and the one by AutoBridge}
    \label{fig:soda_dcp}
\end{figure}

Finally, we present the stability of the timing quality of AutoBridge on both U250 and U280, by increasing the number of kernels from 1 to 8.

\begin{itemize}
    \item Figure~\ref{fig:soda_u280} shows the experiment results on U280. Note that in the default mode, Vivado has very unstable results. Most design points directly failed in routing due to routing resource conflict. In comparison, with the help of AutoBridge, the achieved frequency stays around 300 MHz for up to 6 kernels. 
    
    \item Observe that starting from the 7-kernel design, there is a frequency meltdown (though much better than routing failure). This is because starting from the 7-kernel design, two kernels have to be squeezed into the same region, thus causing more local congestion. In comparison, the U250 FPGA which is larger and has a 2$\times$4 mesh region can hold all the kernels in different regions, leading to a very stable frequency, as shown in Figure~\ref{fig:soda_u280}.
\end{itemize}







\begin{figure}[!h]
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/soda_u280.pdf}
	\caption{Experiment result on U280 FPGA.}
    \label{fig:soda_u280}
\end{figure}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.8\columnwidth]{figures/soda_u250.pdf}
	\caption{Experiment result on U250 FPGA.}
    \label{fig:soda_u250}
\end{figure}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Genome Sequencing (Broadcast Topology)}

We use this benchmark to demonstrate adding latency to shared-memory-based designs, as presented in Section~\ref{sec:shared_memory}.

\begin{itemize}
    \item We choose the Minimap2 accelerator~\cite{guo2019hardware}, which has a broadcast topology as shown in Figure~\ref{fig:minimap_arch}. We can easily adjust the size of each PE by setting certain parameters of the design.
    %The advantage of this design is that we can easily adjust the size of each PE by adjust the \texttt{back\_search\_count} parameter of design.
    
    \item We first use AutoBridge to do the floorplanning and insert registers in RTL for signals that cross the region boundaries. As introduced in Section~\ref{sec:impl_details}, we will manually insert empty modules to the HLS source code to introduce additional registers. These empty modules will be later removed from the generated RTL. 
    
    \item Since this design has statically determined behaviour, we can study if the added registers are hurting the performance by analyzing the HLS report. Comparing the HLS reports, we see that adding three registers to all interfaces of each PE will result in a 2\% performance degradation, which comes from the elongated depth of the pipeline that interacts with the buffers, which is acceptable if we can have huge frequency boost.
    
    \item Table~\ref{tbl:minimap} shows the statistics of the four experiments we run. As can be seen, with the original size of the PE which is small, Vivado can do a decent job. However, when we double the size of each PE, AutoBridge is significantly better.
\end{itemize}



%As every PE in this design conforms to our criteria that BRAM accesses should be within a pipelined environment, we are able to add registers to all interface signals of the PE (and make the internal modifications accordingly), thus moving the PE far away from other parts. 

\begin{figure}[!h]
	\centering
	\includegraphics[width=\columnwidth]{figures/minimap_arch.pdf}
	\caption{Topology of the Minimap2 accelerator}
    \label{fig:minimap_arch}
\end{figure}



\begin{table}[!h]
\caption{Experiment result of genome sequencing on U250}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
         & Fmax (MHz) & LUT \%   & FF \%   & BRAM \% & DSP \% \\ \hline
Default   & 265        & 25.43 & 16.12 & 17.21 & 4.38 \\
AutoBridge    & 267        & 25.48 & 16.29 & 17.21 & 4.38 \\ \hline
Default 2$\times$size & 131        & 38.89 & 23.11 & 17.21 & 8.54 \\
AutoBridge 2$\times$size  & 206        & 38.91 & 23.31 & 17.21 & 8.54 \\ \hline
\end{tabular}%
}
\label{tbl:minimap}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Systolic Array (Mesh Topology)}

We use this benchmark to demonstrate that 1) the correctness of our re-balancing algorithm as introduced in Section~\ref{sec:rebalance} and 2) AutoBridge helps spread medium-size designs evenly across different regions, leading to lower local congestion.

\begin{table}[!h]
\caption{Experiment results of systolic array}
\resizebox{\columnwidth}{!}{%
\begin{tabular}{cccccc}
\hline
\multicolumn{1}{c}{} & \multicolumn{1}{c}{Fmax (MHz)} & \multicolumn{1}{c}{LUT \%} & \multicolumn{1}{c}{FF \%} & \multicolumn{1}{c}{BRAM \%}     & \multicolumn{1}{c}{DSP \%} \\ \hline
Default U280            & 209                         & 34.56                   & 28.95                  &  61.66 & 35.51                   \\
AutoBridge U280             & 323                         & 34.17                   & 28.10                   &  72.67 & 35.51                   \\ \hline
Default U250            & 216                         & 30.04                   & 24.54                  & 26.43                        & 26.15                   \\
AutoBridge U250             & 329                         & 29.83                   & 24.07                  & 26.41                        & 26.15                   \\ \hline
\end{tabular}%
}
\end{table}

\begin{itemize}
    \item Figure~\ref{fig:polysa_arch} shows the topology of our experiment systolic array generated by the PolySA compiler~\cite{cong2018polysa}. Note that while the PE array has a regular shape, the three DDR controllers are located at different dies. Therefore, it is non-trivial to generate a suitable floorplanning of the seemingly regular systolic array.
    
    \item We generate a medium-size 10$\times$8 systolic array targeting U250. We deliberately control the size of the design such that it could barely fit into one die. Figure~\ref{fig:polysa_dcp} shows the difference of the default implementation and the one with AutoBridge. The three colored blocks in the middle are the three DDR controllers. The long orange block on the right is the Vitis platform IP. In the default one, the whole design is packed densely together, while the bottom part of the FPGA is left unused. 
    
    \item In comparison, AutoBridge helps spread the design evenly across the 4 disjoint regions on the left. Note that as this design is relatively small and there are abundant potential places to add registers, we deliberately lower the maximum regional utilization ratio to around 60\% to make the design spread more widely. 
    
    \item Every single edge in the systolic array has reconvergent counterparts, thus it a good candidate to test our re-balancing algorithm. We compare the ratio of improved frequency against the ratio of improved throughput to examine if our modification has impacted the total cycle count. In the U250 version, there are 373 FIFOs (edges) in total. The floorplanning step adds an average of 2.05 cycles of latency to 78 FIFOs. The re-balance step adds an average of 6.82 units depth to 50 FIFOs. To test the performance, we reduce the frequency of the AutoBridge version to the same as the default baseline, and obtain the same throughput as the original design by on-board test (less than 1\% difference).
    
    \item On the U280 experiment, the AutoBridge version uses 0.1$\times$ more BRAM. We found that some IO modules are synthesized with more BRAMs, possibly because we disable the hierarchy rebuild process in synthesis. Still, AutoBrige brings 1.55$\times$ frequency improvement. %Moreover, such large increase is uncommon {jie comapared to what?}.
\end{itemize}









%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Graph Processing (Mixed Topology)}

In this subsection, we demonstrate the effectiveness of our latency analysis from Section~\ref{sec:steal}.

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.9\columnwidth]{figures/pagerank_arch.pdf}
	\caption{Topology of one set of the graph processing units. The U250 design has 4 such sets, and the U280 design has 8 such sets. There is also a central controller not shown here.}
    \label{fig:pagerank_arch}
\end{figure}


Our graph processing design traverses edges of the input graph and updates the vertex attributes accordingly. Figure~\ref{fig:pagerank_arch} shows a local view of parts of the design. Each DDR controller is connected with a set of modules to enable parallel processing. %There is also a central task scheduler not shown. 
The design on U250 has 4 sets of processing units and the U280 one has 8 sets.

As can be seen, every edge in this design belongs to at least one dependency cycle in the topology. 
However, our analysis based on Section~\ref{sec:steal} will lead to a completely different conclusion: there does not exist any pair of reconvergent paths to balance nor dependency cycles in this Figure~\ref{fig:pagerank_arch}. This is due to the following reasons: 1) Every FIFO is accessed in different pipeline loops. 2) Most FIFO accesses are non-blocking  and do not contribute to any dependence cycle or reconvergent path.

In our 8-PE-set experiment on U280, there are 143 FIFOs (edges) in total. AutoBridge adds an average of 2.74 cycles of latency to 89 FIFOs; and no edge is added for re-balacing. To test the performance, we reduce the frequency of the AutoBridge version to the same as the default baseline, and obtain the same throughput as the original design by on-board test (less than 1\% difference).

%Multiple PEs have duplex communication with the centralized controller to obtain information about the vertices of the target graph. Meanwhile, each PE talks to one DDR controller to fetch the information about the edges of the target graph.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \subsection{Summary}

% In this section we present the details of AutoBridge, and frequency improvements of four  benchmarks on two FPGA architectures respectively. By on-board testing we verify that our modifications are correct and does not impair the throughput of the design.

==> src/intro_old.tex <==
\iffalse
Modern FPGAs are continuously developing towards heterogeneous architectures~\cite{url-ultrascale}. To incorporate more resource on-chip, FPGAs are integrating multiple dies on the same interposer. Meanwhile, specialized large scale IPs are being integrated with the programmable logic. Many have fixed locations near dedicated I/O banks (e.g. DDR controller, DMA), and many are even fixed ASIC blocks (e.g. HBM controller, PCIe block).  Figure~\ref{fig:fpga_arch} shows three representative FPGA architectures~\cite{url-alveo}. Such architecture changes significantly reduce the flexibility of programmable fabric.  


\begin{figure}[!bth]
	\centering
	\includegraphics[width=\columnwidth]{figures/fig_FPGA_arch.png}
	\caption{Three representative FPGA architecture}
    \label{fig:fpga_arch}
\end{figure}

%The latest architecture features of FPGAs have profound influences on the compilation stack from user C++ source code to the final bitstream:

\begin{itemize}
    \item First, the programmable logic on the modern FPGAs will be split into discontinuous regions. On the one hand, it is well known that crossing die boundaries incurs additional delay penalty; on the other hand, \todo{} it's less understood that the large IPs will take away significant programmable resources at their fixed locations, also effectively forming non-trivial delay discontinuity. For example in Figure~\ref{fig:fpga_arch}, die boundaries form horizontal gaps and DDR controllers form vertical gaps for the Xilinx U250 FPGA. Global signals passing through the gaps are likely to become timing bottlenecks.
    
    \item Second, IPs with fixed locations may introduce additional critical paths. The Xilinx HBM controller IP is one classic example. It exposes 32 independent interfaces to access external memory, but all at the bottom side of the FPGA, as shown in Figure~\ref{fig:fpga_arch}. Consequently, user logic may be placed in a unbalanced way, with regions near certain IPs packed densely while regions far away left under-utilized. Meanwhile, for modules that are connected to the HBM but fail to be squeezed into the bottom region, their cross-region connection with the HBM will also become critical paths.
\end{itemize}

% The programmable logic on the modern FPGAs is usually split into multiple \textit{disjoint} regions by certain ``gaps'' on modern FPGAs. 
% In general, there are two types of gaps: 
% \begin{itemize}
%     \item First, the die boundaries in multi-die FPGAs. To incorporate more resource on-chip, FPGA vendors integrate multiple dies on the same interposer. However, die-crossing will impose significant delay penalty to signals~\cite{hahn2014cad, nasiri2015multiple}. Moreover, only a limited number of signals can travel across die boundaries.
%     \item Second, the specialized IPs (e.g., DDR controller, PCIe blocks). These modules are usually fixed at certain locations on-chip depending on how the I/O and the motherboard are designed.
% \end{itemize}
% As a result, the usable programmable logic is often split into physically disjoint \textit{regions}.

 %As an example, the Xilinx U250 FPGA is split into 8 disjoint regions by die boundaries and the array of DDR controller IPs. Meanwhile, the U280 FPGA with all HBM ports at the bottom is likely to cause unbalanced utilization ratio.

\todo{complain -> motivation and challenge}
\todo{HBM IP at intro too detailed}
\todo{challenge: hard to predict }
\todo{a bigger problem on large FPGAs}
\todo{harden IP}
\todo{blockage}
\todo{congestion -> unroutable}
\todo{contribution too detailed}
\todo{region-aware coarse floorplanning}
\todo{FSM dataflow network -> conflict}
\todo{make a name}
\todo{cut-set retiming -> confusing}
\todo{define the problem}
\todo{related work -> end}
\todo{map schematic and dcp}
\todo{motivation example show why RTL not working}
\todo{make sense for RTL but not for HLS}
\todo{section 5 correlates to motivation example}
\todo{first FIFO, then extend to other interfaces}
\todo{couple floorplanning and pipelining}
\todo{floorplaninig -> additinal constraint -> pipelining signals}
\todo{high level objective}
\todo{insert additional register}
\todo{introduce the next question}

\todo{contribution -> specific context, similar to DAC}
\todo{two problems and results, on average}
\todo{problem formulation combined with examples}


The current FPGA automation stack are not catching up with the architecture advancements. The high-level synthesis compiler at the front end, which compiles C++ source code into RTL designs, often produces global signals whose wire delay are underestimated~\cite{guo2020analysis}. This is because HLS knows nothing about the final location of each module, so it cannot determine how much register to put on the signals connecting two modules. The HLS compiler also lacks architecture-level information, such as where the DDR controllers are. As a result, although HLS can guarantee a low combinational delay for signals, the wire delay is beyond control and will be further degraded by the die boundaries and potential IP barriers.

At the back end, the floorplanning and placement tools are limited in their capability to deal with the challenges without the front-end support. On one hand, the additional delay penalty from die boundaries and IP barriers does not fit well with the traditional tools that minimize wire lengths, which are designed for continuous and uniform programmable fabric. Some tools attempt to address this issue by heuristics to pack logic densely within regions in favor of region crossing~\cite{hahn2014cad, nasiri2015multiple}, but at the cost of local congestion. On the other hand, the location constraints of embedded IPs often force signals to travel long distance, but the physical design tools do not have the flexibility to arbitrarily insert registers, as they must obey the input cycle-accurate speculation imposed by the HLS scheduling phase.

To address the dilemma, we propose cross-stack solutions to optimize floorplanning and HLS compilation together. We make the floorplaner interact with the HLS scheduler, passing spatial information to the scheduler, who in turn adjusts the generated RTL to fit the need of the floorplaner. The cross-stack interaction works in the following way:

%\todo{equivalence, solution space, what is acceptable solution, the metric, don't define the problem using the solution, no approaches in problem definition, what is legal, relate the previous works to the problem definition, modify both physical space and the scheduling space, do we start with existing solution or c program without any solution? }



\begin{itemize}
    \item The floorplaner attempts to spread the design across the whole chip, with the priority to balance \textit{local} congestion.
    \item Based on the tentative floorplan, the HLS scheduler increases the register level for signals that span long distances to remove \textit{global} critical paths.
    \item The HLS scheduler analyzes if the increased latency on certain signals will impact the overall performance, and instruct the floorplaner that certain modules must be arranged close to each other.
    \item The final floorplan will be used to override the default behavior of the physical design tool to improve the achievable frequency.  
\end{itemize}




%Specifically, our problem is formulated as follows. Given an HLS C++ program $P$, which includes a set of functions $F$. Each HLS function $f \in F$ has a resource requirement, which excludes all sub-functions called in $f$. Meanwhile, each function $f$ will be compiled into an Verilog module $v$. For a pair of functions $(f_1, f_2)$, their corresponding Verilog modules $(v_1, v_2)$ will have direct wire connection if $f2$ is invoked within $f1$, or if they both The target FPGA is split into a set of regions $R$, and the available resource of each region $r \in R$ is known. The goal is to assign each $f \in F$ to one of the region $r \in R$ such that 1) the resource utilization of region $r_i$ is below a given threshold $MaxUsageRatio_i$, and 2) for any pair of functions $(f_1, f_2)$, if $f1$ has direct signal connection with $f2$ and $f1$ and $f2$ are assigned to different regions, then   

%One challenge is how to absorb the additional registers in global signals, which will result in extra latency and may hurt correctness and performance. Our approach tackles this challenge at HLS level, as modifying register count for signals based on C++ source code has unique advantages. First, the compiler will automatically adjust the surrounding logic to adapt to the latency change, thus correctness can be guaranteed. Second, performance analysis is easy as we have the complete state transition information of the internal operations of each module. Therefore, we can locate positions whose latency is irrelevant to the overall throughput. 

One challenge is to analyze the performance impact if the scheduler increases the buffer level for certain signals, especially in dataflow designs. In essence, an HLS dataflow design is an FSM dataflow network~\cite{peng1991data}, where multiple parallel finite state machines (FSM) communicate through FIFOs. While it will be functionally correct to use multiple concatenating FIFOs to bridge long distances, the additional latency between a pair of parallel FSM may hurt the overall throughput. Currently, the throughput analysis for FSM dataflow network is still an open question due to the significant expressiveness of the model. However, in this work, we propose methods based on cut-set retiming~\cite{sykung} to ensure that our additional buffer will not decrease the throughput from that of the original design. As the technique works on acyclic graphs, we further identify special cases where we can resolve cycles in the dataflow graph. Finally, to minimize the area overhead, we formulate the problem as a multi-min-cut problem and propose a polynomial-time algorithm for exact solution.


% \begin{itemize}
%     \item For modules communicating through shared memory, it will be hard for RTL-level approaches to systematically insert registers without causing errors. However, at C++ level we could instruct HLS compilers to add additional registers, then let the compiler automatically adjust the surrounding logic to ensure the same overall functionality. 
    
%     \item For dataflow designs where modules communicating through FIFO interfaces, we propose a polynomial-time algorithm to adjust the configuration of FIFO depths to re-balance the reconvergent paths, which makes sure that the throughput after buffer insertion is the same as before. Moreover, we utilize the scheduling information of each dataflow module to identify special cases where we can more aggressively add registers.    
% \end{itemize}

% \begin{figure}[!h]

% \centering
% \includegraphics[width=\columnwidth]{figures/transform.png}
% \caption{Convert cycles to reconvergent paths if the write operation is upstream to the read operation in the same pipelined loop.}
% \label{fig:break_cycle}

% \begin{lstlisting}[language=c++,firstnumber=1]
% while (1) { #pragma HLS pipeline II=1
%   ...
%   fifo_a.write(...);
%   HLS_WAIT_CYCLE(2); // change source code for cut-set retiming
%   fifo_b.read(...);
% }
% \end{lstlisting}
% \caption{Shared-memory-based communication}
% \label{code:shared_memory}

% \end{figure}

% figure~\ref{} provides an example where it is much easier to insert buffer at HLS level. In this design, there are three modules communicating through FIFO, and the three FIFOs form a cycle. Assume that module 1 is arranged to be far from module 2 and 3, so that we need to insert additional buffer between module 1 and 2, and between 1 and 3. If working with RTL, it

% Note that while part of our approach with dataflow designs look similar to previous works such as the latency insensitive theory~\cite{carloni2001theory}, our problem is different and we have our own contribution. First, our approach also supports other types of interfaces, such as shared memory. Previous works have studied how to determine from scratch the required FIFO depth for latency insensitive system, whose control flow is independent of the data. However, in many HLS designs the FIFO operations are conditional on the actual input data. Therefore, in our case we choose to rely on the initial configuration of FIFO depth from users and only perform the necessary adjustment. We guarantee that after our buffer insertion and corresponding adjustment, we will not lose throughput compared to the original design. Moreover, our adjustment algorithm runs in polynomial time, while it is NP-hard to determine the optimal depth from scratch. Therefore, our contribution is orthogonal to previous works. \todo{add citation}

%Although there are previous works studying how to insert additional registers to break critical paths, such as the latency insensitive theory~\cite{carloni2001theory}, our problem and approach are different. First, we will show that if we simply add registers without providing corresponding floorplan constraints, the final frequency can be barely improved. Second, our work focus on adding extra latency based on the scheduling information from the HLS compiler, which is less studied.  

%In comparison, we will have much more limitation in adding registering to RTL source code. To ensure correctness, we will be limited to designs with special interfaces like FIFO. Previous approaches such as the latency-insensitive theory~\cite{carloni2001theory} impose strict assumption about the behaviour of the FIFO interfaces. For example it assumes that every cycle the outbound FIFO interface must produce a data and every inbound FIFO interface must consume a data. Thus the analysis will be much more coarse-grain as the internal of modules are treat like black-boxes. And again, for other designs that do not use FIFO interfaces, it is extremely difficult to systematically insert registering without break the functionality.

In summary, the technical contributions of this paper are as follows:

\begin{itemize}
    \item We propose to co-optimize the HLS compilation and floorplanning to address the timing issue on gigantic multi-die FPGAs with large fixed/hard IPs.
    \item We propose scalable methods to floorplan the HLS designs that pareto-optimally balance local utilization ratio and minimize total count of region crossing signals. 
    \item For FSM dataflow network, we propose polynomial-time algorithms to adjust the FIFO configuration without throughput loss, while minimizing area overhead.
    \item We implement the tool, AutoBridge, that works transparently with Vivado HLS. With processing time in the order of seconds, AutoBridge significantly improves the maximum frequency of large-scale designs. In some cases, we make the originally unroutable designs achieve more than 300 MHz. 
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Motivation Example}

We first show the implementation of a medium-size neural network accelerator (762 BRAM18K, 3200 DSP48E, 502K FF, 432K LUT), as shown in Figure~\ref{fig:polysa_arch}. In theory, such regular mesh structure is supposed to be FPGA-friendly. However, due to the fixed locations of DDR controllers and the heuristics used in placement to avoid region crossing, the actual implementation is highly irregular, as shown in Figure~\ref{fig:polysa_dcp}. The high local utilization in the 3rd die results in routing congestion. With the default Vivado tool set, this design runs at 216 MHz on the U250 FPGA. 

In comparison, our tool arranges the systolic array such that each region has a limited resource usage ratio of 60\%. Based on our observation about the fixed DDR controllers, we constrain that the user logic should not overlap with the DDR controllers. Meanwhile, all connection signals across different regions have been adequately registered to remove global critical paths. The optimized version achieves 329 MHz, a 53\% improvement in frequency. On-board experiments confirm that the throughput is also not affected, where we deliberately decrease the clock frequency to be the same as the baseline, and compare the performance of the baseline and the optimized version.

%This implementation has two kinds of timing issue. First, the high local utilization in the 3rd die results in routing congestion. Second, the location constraints of DDR controllers force some neighboring PEs to actually be far away, but their interconnects are not adequately pipelined, as the HLS has no idea of the final layout of the design. With the default Vivado tool set, this design runs at 216 MHz on the U250 FPGA. 



\begin{figure}[!h]
    \centering
    \includegraphics[width=0.6\columnwidth]{figures/polysa_arch.pdf}
    \caption{Topology of the systolic array with 3 DRAMs.}
    \label{fig:polysa_arch}
\end{figure}

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.6\columnwidth]{figures/polysa_dcp.png}
	\caption{Comparison of the default floorplan of the 10x8 systolic array on U250 and the one by AutoBridge}
    \label{fig:polysa_dcp}
\end{figure}

Another stencil processing design on the U280 FPGA highlights how our approach facilitates region crossing. This design features four Jacobi-2D kernels chained in a linear topology (512 BRAM18K, 2816 DSP48E, 465K FF, 240K LUT). In figure~\ref{fig:soda_dcp}, each color represents one Jacobi2D kernel. In the baseline design generated by Vivado, the 4 kernels are twisted together. Each kernel spans across the die boundary and the middle gap multiple times. In comparison, AutoBridge keeps each individual module in the same region, and adds additional pipelining to the wires connecting them to facilitate region crossing. While the design originally failed in routing by default Vivado settings, AutoBridge makes it achieve 297 MHz.

\begin{figure}[!h]
	\centering
	\includegraphics[width=0.7\columnwidth]{figures/soda_dcp.png}
	\caption{Comparison of the default floorplan of the 4-kernel stencil accelerator on U280 and the one by AutoBridge}
    \label{fig:soda_dcp}
\end{figure}


%As shown in the right part of Figure~\ref{fig:polysa_dcp}, for the same systolic array design, our approach distributes the design evenly across the left regions of the 4 dies, which significantly lowers the local congestion level and avoids the resource contention between user logic and the DDR controller. Meanwhile, for neighboring PEs that are placed into different regions, we adequately insert buffers into the interconnect, so that region-crossing is no longer a problem.



\fi




